Postselection-free experimental observation of the measurement-induced phase transition in circuits with universal gates

Monitored many-body systems can exhibit a phase transition between entangling and disentangling dynamical phases by tuning the strength of measurements made on the system as it evolves. This phenomenon is called the measurement-induced phase transition (MIPT). Understanding the properties of the MIPT is a prominent challenge for both theory and experiment at the intersection of many-body physics and quantum information. Realizing the MIPT experimentally is particularly challenging due to the postselection problem, which demands a number of experimental realizations that grows exponentially with the number of measurements made during the dynamics. Proposed approaches that circumvent the postselection problem typically rely on a classical decoding process that infers the final state based on the measurement record. But the complexity of this classical process generally also grows exponentially with the system size unless the dynamics is restricted to a fine-tuned set of unitary operators. In this work we overcome these difficulties. We construct a tree-shaped quantum circuit whose nodes are Haar-random unitary operators followed by weak measurements of tunable strength. For these circuits, we show that the MIPT can be detected without postselection using only a simple classical decoding process whose complexity grows linearly with the number of qubits. Our protocol exploits the recursive structure of tree circuits, which also enables a complete theoretical description of the MIPT, including an exact solution for its critical point and scaling behavior. We experimentally realize the MIPT on Quantinuum's H1-1 trapped-ion quantum computer and show that the experimental results are precisely described by theory. Our results close the gap between analytical theory and postselection-free experimental observation of the MIPT.

==> extras/extras.tex <==
\begin{figure}[ht!]
    \centering

    % First subfigure
    \begin{subfigure}{0.48\textwidth} % width of the subfigure
        \begin{quantikz}
            \lstick{$\rho$} && \ctrl{1} &\\
            \lstick{$\ket{0}$} & \gate{R_Y (\theta)} & \targ{} & \meter{}
        \end{quantikz}
        \caption{Standard weak measurement circuit.}
        \label{fig:standard-weak-measurement-circuit}
    \end{subfigure}
    \hfill
    \hfill% adds space between subfigures

    % Second subfigure
    \begin{subfigure}{0.48\textwidth}
        \begin{quantikz}
            \lstick{$\rho$} & \gate[2]{ZZ(\phi)} & &\\
            \lstick{$\ket{+}$} & & \gate{R_X (\frac{\pi}{2})} & \meter{}
        \end{quantikz}
        \caption{Native weak measurement circuit.}
        \label{fig:native-weak-measurement-circuit}
    \end{subfigure}

    % Main figure caption
    \caption{Two weak measurement circuits, where $\phi \equiv \pi/2 - \theta$. The qubit encoding $\rho$ comes from the quantum tree, while the bottom qubit is an ancillary qubit to implement the weak measurement. Circuit~\ref{fig:standard-weak-measurement-circuit} is the standard one for performing the weak measurement. Ignoring a global phase, Circuit~\ref{fig:native-weak-measurement-circuit} is logically equivalent to Circuit~\ref{fig:standard-weak-measurement-circuit} but uses the native two-qubit gate for the Quantinuum H1-1, defined as $ZZ(\phi) \equiv \exp{\left(-i(Z \otimes Z) \phi / 2\right)}$.}
    \label{fig:weak-measurement-circuits}
\end{figure}

We provide intuition here, and the interested reader can follow the details in Appendix~\ref{appendix:reverse_map}, where we treat the problem using both the root and probe qubits. Here though, we focus on the case of just the root qubit. In the expansion process of the dynamical quantum tree, the root qubit begins in the state $\rho_{\mathrm{root}} =  \mathbb{I}/2$. Given a set of unitaries $\mathcal{U}$ and weak measurement outcomes $M_w$, one can define an effective $(2^{2^t}, 2)$ matrix $T_t \equiv T_t(\theta, \mathcal{U}, M_w)$ that maps $\rho_r$ to a final state on all $2^t$ qubits of the system. Such a state will evolve as:
\begin{equation} \label{eq:root-qubit-evolved}
    \rho_{\mathrm{tot}} = \frac{T_t \rho_{\mathrm{root}}  T_t^{\dagger}}{\Tr{\left[ T_t \rho_{\mathrm{root}}  T_t^{\dagger}\right]}}
    = \frac{T_t T_t^{\dagger}}{\Tr{\left[ T_t  T_t^{\dagger}\right]}}.
\end{equation}

Now suppose we instead consider the collapse process of the dynamical quantum tree model in Figure~\ref{fig:collapse-tree-diagram}. The initial state is $\rho_0 = \mathbb{I}/2$ for each input to the leaf nodes of the tree in Figure~\ref{fig:collapse-tree-diagram}, and the state evolves using the matrix $T_t^{\dagger}$. We therefore find:
\begin{equation} \label{eq:collapse-process-evolution}
    \rho_t(\theta, \mathcal{U}, M_w) = \frac{T_t^{\dagger} \rho_0^{\otimes 2^t}  T_t}{\Tr{\left[ T_t^{\dagger} \rho_0^{\otimes 2^t}  T_t\right]}} = \frac{T_t^{\dagger} T_t}{\Tr{\left[ T_t^{\dagger}  T_t\right]}}.
\end{equation}
Note that $T_t$ has at most two non-zero singular values, therefore the same is true for $T_tT_t^{\dagger}$ and $T_t^{\dagger}T_t$. Furthermore, notice that the purity of $\rho_{\mathrm{tot}}$ and $\rho_t$ are identical:
\begin{equation} \label{eq:purity}
    \Tr{\left[ \rho_t^2 \right]} = \frac{ \Tr{ \left[ T_t^{\dagger} T_t T_t^{\dagger} T_t \right]}}{\left(\Tr{\left[ T_t  T_t^{\dagger}\right]}\right)^2} = \frac{ \Tr{ \left[ T_t T_t^{\dagger} T_t T_t^{\dagger} \right]}}{\left(\Tr{\left[ T_t  T_t^{\dagger}\right]}\right)^2} = \Tr{\left[ \rho_{\mathrm{tot}}^2 \right]},
\end{equation}
where we make use of the cyclic property of the trace again. Since the purity of $\rho_t$ determines $Z_t(\theta, \mathcal{U}, M_w)$, we find that the purity of both states yields the same estimate for $Z_t(\theta, \mathcal{U}, M_w)$.
